On the Automated Synthesis of Enterprise Integration Patterns to Adapt Choreography-based Distributed Systems

The Future Internet is becoming a reality, providing a large-scale computing environments where a virtually infinite number of available services can be composed so to fit users' needs. Modern service-oriented applications will be more and more often built by reusing and assembling distributed services. A key enabler for this vision is then the ability to automatically compose and dynamically coordinate software services. Service choreographies are an emergent Service Engineering (SE) approach to compose together and coordinate services in a distributed way. When mismatching third-party services are to be composed, obtaining the distributed coordination and adaptation logic required to suitably realize a choreography is a non-trivial and error prone task. Automatic support is then needed. In this direction, this paper leverages previous work on the automatic synthesis of choreography-based systems, and describes our preliminary steps towards exploiting Enterprise Integration Patterns to deal with a form of choreography adaptation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{Jos\'{e} Proen\c{c}a and Massimo Tivoli (Eds.):\\
14th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'15)\\
EPTCS 201, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.201.3}{10.4204/EPTCS.201.3}}
\pdfoutput=1

